Debiasing Algorithm through Model Adaptation

Large language models are becoming the go-to solution for the ever-growing number of tasks. However, with growing capacity, models are prone to rely on spurious correlations stemming from biases and stereotypes present in the training data. This work proposes a novel method for detecting and mitigating gender bias in language models. We perform causal analysis to identify problematic model components and discover that mid-upper feed-forward layers are most prone to convey bias. Based on the analysis results, we intervene in the model by applying a linear projection to the weight matrices of these layers. Our titular method, DAMA, significantly decreases bias as measured by diverse metrics while maintaining the model's performance on downstream tasks. We release code for our method and models, which retrain LLaMA's state-of-the-art performance while being significantly less biased.

==> figures/dama_schema.tex <==
\begin{figure}[t]
     \centering
     \begin{subfigure}[tb]{0.45\textwidth}
         \begin{subfigure}[tb]{\textwidth}
            %\vspace{0.45cm}
             \centering
             \vspace{0.5cm}
             \text{``The \textcolor{schema_celadon}{\textbf{lifeguard}} laughed because \textbf{\_\_\_}''}
             \vspace{0.5cm}
             \caption{Stereotypical prompt}
             \label{fig:dama_prompt}
             \vspace{0.5cm}
        \end{subfigure}
        \begin{subfigure}[tb]{\textwidth}
             \centering
             \includegraphics[width=\textwidth]{figures/DAMA_Layer_diagram.png}
             \vspace{0.25cm}
             \caption{\dama{} intervention in each layer}
             \label{fig:dama_intervention}
         \end{subfigure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[tb]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Projections_DAMA.png}
         \caption{Projections}%a sterotypical key vector to a plain spread by gender vectors. Without and with \dama{}}
         \label{fig:dama_projection}
    \end{subfigure}
    \hfill
    \begin{subfigure}[tb]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/DAMA_probabilities.png}
         \caption{Output probabilies}
         \label{fig:dama_probabilities}
     \end{subfigure}

     \caption{Schema depicting \dama{} intervention in LLaMA model layer (b). 
             We show the behavior of the model when presented with a stereotypical prompt, suggesting the usage of the male pronoun (a). Figure (c) shows the projections of the feed-forward latent vectors onto output space. With \dama{} (lower part), we nullify the biased factor of the representation. It results in balanced probabilities of pronouns in the model's prediction, as shown in Figure (d).}
     \label{fig:dama_schema}
\end{figure}

==> sections/01b_introduction_with_comments.tex <==
\section{Introduction}


\jana{OK a more higher-level comment. This is more a "Reviewer 2" comment, as I'm not an expert on debiasing. But I just skimmed the Abstract, Intro and Related Work and you don't give much related work on debiasing and don't relate to it. In my (very high level and fuzzy) knowledge, there is literature on debiasing. How is your work novel compared to that work?}

% The recent advent of Large Language Models offers promises\jana{Eh... offers promises - has potential to improve a wide variety...} of improvements for a wide variety of NLP tasks.
% However, 

Large language models have a large capacity for learning linguistic and factual information from training data, but they are prone to capture unwanted biases. % stemming from training data.
%One example of such bias is related to gender. 
It has been shown that LLMs are, to a varying 
extent, gender biased \citep{stanczak_survey_2021, blodgett_language_2020}.\jana{Are there more refs, maybe?}
This bias is manifested by relying on a spurious correlation between seemingly gender-neutral expressions or words and specific gender.
For instance, 
%the\od{no article}
language models tend to ascribe stereotypical gender to certain practitioners, such as ``male mechanics'' or ``female cleaners'' \citep{lu_gender_2019}. 
In many tasks, the models also show uneven performance for the test examples involving different gender contexts.

In this work, we analyze the \llama{} family of models \citep{touvron_llama_2023}.
These openly available models obtain state-of-the-art performance on a variety of downstream tasks.
We focus specifically on the gender bias present in these models.\jana{Why only gender? Although it is not, it may seem as an arbitrary decision. Maybe either say "because of its particular pervasiveness and impact", "because it is particularly pervasive and harmful" idk; or, if possible, you can add "but our method is applicable to other biases".}
We specifically ask: 1) Can we identify evidence of gender bias in \llama{}?
%Are \llama{} models gender-biased?\jana{Well, duh, yes I bet! Can we reframe the question so it does not sound so trivial... "Does the ubiquitous gender bias pertain to llama models?" or better yet "Can we identify evidence of gender bias in llama?" (like we half expect it to be there based on the literature, we're just going to find the evidence)} 
Specifically, do they associate professional names with their stereotypical gender?
2) Can we identify which components of the model store the gender-biased representation?
3) Can we edit the model's weights to decrease the bias while preserving its performance on other tasks? 
\jana{Yup, I found it: Inanimate objects cannot be possessive: https://writingcenter.uagc.edu/possessives ("Do not form the possessive of an inanimate object; use an adjective or an "of" phrase.")}
   

% To approach this problem, we investigate the following aspects of the language model's handling of gender representation: 1) Is it possible to identify components responsible for biased generation in causal language modeling? 2) Can we distinguish components conveying factual gender signals (e.g., connected to gendered nouns) from once emitting bias associated with stereotypical gender roles? 3) Is it possible to edit specific components in order to decrease the overall gender bias of the model's predictions while preserving good performance on its original task?

To answer the first question we check the \llama{} performance on popular tests for gender bias: \wb{} \citep{zhao_gender_2018} and \stereos{} \citep{nadeem_stereoset_2021}. 
We further introduce our interpretable metric that evaluates bias on the original task of language generation.
%introduce our interpretable gender bias evaluation method in language generation.\jana{Swap the order. Start with the standard measures (second sentence) and only THEN, in the second sentence, add "We additionally introduce our own interpretable gender bias evaluation method, which ... (why? what does it have that the standard ones do not)? The reason for switching is that (1) Having your own method sounds shady, so establish your soundness by giving the standard methods first. (2) Your new evaluation method needs to relate to the standard methods, hence, goes second. (3) This looks like yet another goal/contribution of the paper. So I'm imagining you start the paragraph with the popular test and from there, you launch to introduce your metric.}
To answer the second question, we perform causal tracing \citep{vig_causal_2020, meng2022locating}.
We monitor changes in the distribution of predictions when the stereotypical representation is revealed only in one of the components such as MLP or attention layer.
\david{It is one of the MLPs, so shouldn't it be "an MLP"? Also, this is the first occurence of the abbrev. MLP, it is well known, but anyway, we could add (multilayer perceptron) in brackets.}
\jana{Why only in your metric and not the other metrics? Is your metric an inherent part of the DAMA method actually? If so, this section needs reformating with focus primarily on DAMA and secondarily on the metric as part of it. If the metric is standalone, it probably needs a tiny little bit of introduction and motivation, maybe a name of its own? I don't like "our metric", sounds fishy.}
\od{I don't have a problem with your own metric (or even with it going first), but it obviously needs to be rooted + evaluated itself, and you need to point it out}
Following the terminology of \citet{pearl_direct_2001}, we call such component \emph{gender bias mediator}.
% \david{What components?}

To tackle the last question we introduce ``\emph{Debiasing Algorithm through Model Adaptation}''.
In \dama{}, we edit bias-vulnerable feed-forward layers by multiplying linear transformation weights by the orthogonal projection matrix similar to \citet{ravfogel_linear_2022}.\jana{I'm confused. In Abstract, you say "applying linear projection to the output of these layers" (so not changing the original weights, right?) But later in Intro you say "In DAMA, we edit bias-vulnerable by multiplying linear transformation weights...", so do you actually edit the weights in place or replace the layers with something else? In the first case, I imagine applying (stacking) subsequent transformation AFTER the vulnerable layers without any change to them; in the second case, the word edit suggests some kind of retraining or fine-tuning of some sort of the actual weights. If you could unify that, that would help me.}
Our results show that with directed changes in model weights, we can reduce gender bias substantially while having only a minimal impact on the model's performance.
Specifically, we monitor changes in language modeling (measured by perplexity) and four language understanding downstream task performance.

To summarize, our contributions are as follows:
We evaluate gender bias in \llama{} models and introduce a novel transparent metric quantifying bias directly in language generation;
We identify the MLP in mid-upper layers as the ones responsible for conveying bias;
Lastly and most importantly, we propose \dama{}, a method for editing weights of those layers to significantly reduce bias without sacrificing performance on other tasks.
    

% The paper is structured as follows: in Section~\ref{sec:setup} we describe the details of considered models and evaluation scheme;
%  Section~\ref{sec:tracing} \tomas{3 instead of 3.2?} describes causal tracing, which we use to identify bias-vulnerable components;
%   in Section~\ref{sec:dama}, we present DAMA and proof its effectiveness.
%    Finally, we summarize the related work (Section~\ref{sec:related}) and main findings (Section~\ref{sec:conclusions}).\od{this paragraph could be dropped, it's a 10-page paper, not a thesis}

\jana{This is a nice paper with potential. I think it should go somewhere nice (ICLR is your plan). My main problem is that I'm not explicitly convinced about the actual contribution, although I implicitly sense it is there. First, I don't clearly see the improvement/novelty in context of the previous work (this might be due to my own ignorance I should admit). Second, there seem to be like three contributions which are gradually revealed in the course of Introduction: identifying gender bias in LLama, then suddenly some new metric drops (with that I have probably the greatest problem, but only with the little information you provide about it) and finally DAMA.}
\od{agree, the contributions list should be very explicit -- even going as far as an itemized list}

\input{figures/FF_schemes.tex}

==> sections/93_generation_examples.tex <==
\section{Generation Probabilites}

\input{tables/generation_examples}

==> sections/X2_bias_evaluation.tex <==
\section{Gender Bias Evaluation}
\label{sec:bias-eval}


\subsection{Modeling Bias in Generation}

For core gender bias evaluation in generative models, we use the set of professions\footnote{\url{https://github.com/tolga-b/debiaswe/blob/master/data/professions.json}} annotated by \cite{bolukbasi_2016}. Each profession is assigned two scores: \fact score $x_f$ (originally called \emph{definitionality}) and \stereo score $x_s$. They define how strongly the words are connected with the male or female gender either semantically or through stereotypical cues. By conventions, scores range from $-1$ for female-associated words to $1$ for male ones.\footnote{We use positive values for male gender following the conventions from . This is only an arbitrary choice and choosing opposite polarities wouldn't affect this analysis. Importantly, we do not intend to ascribe negative connotations to any of the genders.}

Based on the model, we can compute the empirical association of words by observing continuations for ... prompts of structure:

\begin{equation*}
X = \text{``The \textbf{plumber} was't paid for the job because...''}
\end{equation*}

Where the \textbf{plumber} is gender neutral and associated with a male bias, we measure the probabilities for gendered prediction for a given prompt $P_M(o|X)$. We use pronouns $o_+ = \text{``he''}$ and $o_- = \text{``she''}$, because they are probable continuations for given prompts and, in English, they carry gendered information.

Subsequently for each profession, we compute \empiric score $y = P_M(o_+|X) - P_M(o_-|X)$. This score is in the same range as \fact ($x_f$) and \stereo scores ($x_s$). Thus we can approximate the effect of those scores on the language model's prediction by linear regression:

\begin{equation}
    y = a_s \cdot x_s + a_f \cdot x_f + b_0
\end{equation}

The coefficients of the linear fit have the following interpretations: $a_s$ is an impact of stereotypical signal on the model's predictions; $a_f$ is an impact of semantics; and the intercept $b_0$ is the general bias of the model. In other words $b_0$ measures how much more probable is the prediction of male than female pronouns for a random professional word when controlling for stereotypical and semantic gender signals.










==> sections/sections_00_abstract.tex <==
\begin{abstract}
Large language models are becoming the go-to solution for the ever-growing number of tasks.
However, with growing capacity, models are prone to rely on spurious correlations stemming from biases and stereotypes present in the training data.
This work proposes a novel method for detecting and mitigating gender bias in language models.
We perform causal analysis to identify problematic model components and discover that mid-upper feed-forward layers are most prone to convey bias.
Based on the analysis results, we intervene in the model by applying a linear projection to the weight matrices of these layers.
Our titular method \dama{} significantly decreases bias as measured by diverse metrics while maintaining the model's performance on downstream tasks.
We release code for our method and models, which retrain \llama{}'s state-of-the-art performance while being significantly less biased.\footnote{The code available at: 
\url{https://github.com/tomlimi/DAMA}}
\end{abstract}

==> sections_00_abstract.tex <==
\begin{abstract}
Large language models are becoming the go-to solution for the ever-growing number of tasks.
However, with growing capacity, models are prone to rely on spurious correlations stemming from biases and stereotypes present in the training data.
This work proposes a novel method for detecting and mitigating gender bias in language models.
We perform causal analysis to identify problematic model components and discover that mid-upper feed-forward layers are most prone to convey bias.
Based on the analysis results, we intervene in the model by applying a linear projection to the weight matrices of these layers.
Our titular method \dama{} significantly decreases bias as measured by diverse metrics while maintaining the model's performance on downstream tasks.
We release code for our method and models, which retrain \llama{}'s state-of-the-art performance while being significantly less biased.\footnote{The code available at: 
\url{https://github.com/tomlimi/DAMA}}
\end{abstract}

==> tables/llama_lm_bias.tex <==
\begin{table}
\centering
\caption{Linear model coefficients for bias in LLaMA models Model's probabilities in linear scale.}
\label{tab:llama_lm_bias}
\begin{tabular}{lrrrr}
\toprule
 & $a_{f}$ & $a_{s}$ & $b$ & $R^2$ \\
Parameters &  &  &  &  \\
\midrule
7 & 0.313 & 0.182 & 0.107 & 0.359 \\
13 & 0.344 & 0.220 & 0.103 & 0.425 \\
30 & 0.333 & 0.204 & 0.134 & 0.365 \\
65 & 0.308 & 0.194 & 0.132 & 0.362 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/llama_lm_bias_log.tex <==
\begin{table}
\centering
\caption{Linear model coefficients for bias in LLaMA models Model's probabilities in log scale.}
\label{tab:llama_lm_bias_log}
\begin{tabular}{lrrrr}
\toprule
 & $a_{f}$ & $a_{s}$ & $b$ & $R^2$ \\
Parameters &  &  &  &  \\
\midrule
7 & 2.626 & 1.244 & 0.816 & 0.575 \\
13 & 2.950 & 1.446 & 0.780 & 0.627 \\
30 & 2.940 & 1.375 & 0.955 & 0.594 \\
65 & 2.729 & 1.385 & 0.970 & 0.602 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/main_results.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{@{}l|cccc|ccc|ccc||c|ccc@{}}
\toprule
            & \multicolumn{4}{c|}{Bias in LM}                     & \multicolumn{3}{c|}{WinoBias}     & \multicolumn{3}{c||}{StereoSet (gen)} & LM   & \multicolumn{3}{c}{Downsteram} \\ 
            & $a_s$ & $a_f$ & $b$    & $R^2$ & Acc    & $\Delta S$ & $\Delta G$ & LM         & ss         & ICAT      & PPL  & ARC-C     & MMLU     & OBQA    \\ \midrule
LLaMA 7B    & 0.235                     & 0.320 & 0.072  & 0.494 & 59.1\% & 40.3\%     & 3.0\%      & 95.2       & 71.9       & 53.7      & 26.1 & 42.2      &          & 57.2    \\
% l9_on_nd256_ncv_val_neutral_delta_only_nw
+ DAMA      & -0.005                    & 0.038 & -0.006 & 0.208 & 57.3\% & 31.5\%     & 2.3\%     & 95.5       & 69.3       & 58.5      & 28.9 & 41.8      &          & 56.2    \\
$\pm$ (std) & 0.004                     & 0.004 & 0.004  & 0.026 & 0.5\%  & 0.9\%      & 0.7\%      & 0.3        & 0.8        & 1.5       & 0.2  & 0.4       &          & 0.5     \\
+MEMIT      & 0.209                     & 0.282 & 0.071  & 0.497 & 59.3\% & 40.5\%     & 3.3\%      & 95.6       & 72.0       & 53.6      & 26.1 &           &          &         \\
% +FT         &                           &       &        &       &        &            &            &            &            &           &      &           &          &         \\ \midrule
LLaMA 13B   & 0.270                     & 0.351 & 0.07   & 0.541 & 70.5\% & 35.7\%     & -1.5\%     & 95.2       & 71.4       & 54.4      & 19.8 & 44.9      &          & 55.4    \\
%l10_on_nd512_ncv_val_neutral_delta_only_nw
+DAMA       & 0.148                     & 0.222 & 0.059  & 0.472 & 66.4\% & 31.1\%     & -1.1\%     & 94.4       & 68.6       & 59.4      & 21.0 & 44.7      &          & 56.2    \\ \midrule
% l17_on_ncv_val_neutral_delta_only_nw
LLaMA 30B   & 0.265                     & 0.343 & 0.092  & 0.499 & 71.0\% & 36.0\%     & -4.0\%     & 94.7       & 68.4       & 59.9      & 20.5 &           &          &         \\
+DAMA       & 0.105                     & 0.172 & 0.059  & 0.471 & 63.7\% & 26.7\%     & -3.7\%     & 94.8       & 65.7       & 65.0      & 19.6 &           &          &         \\ \midrule
%l20_on_nd2048_ncv_val_neutral_delta_only_nw
LLaMA 65B   &   0.249 &  0.316 &  0.095 &   0.490    &   73.3\%     &   35.7\%  &    1.4\%        &            &            &           &    19.5  &           &          &         \\
+DAMA       &                           &       &        &       &        &            &            &            &            &           &      &           &          &         \\ \bottomrule
\end{tabular}
\caption{Performance and bias evaluation for the \llama{} models and their debiased instances.}
\label{tab:main-results}
\end{table}

==> tables/main_results_bias.tex <==
\begin{table}[!th]
\scriptsize
\centering
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
            & \multicolumn{4}{c}{Bias in LM}                     & \multicolumn{3}{c}{WinoBias}     & \multicolumn{3}{c}{StereoSet gender} \\\cmidrule(r){2-5}\cmidrule(lr){6-8}\cmidrule(l){9-11}
            & $\downarrow$ $a_s$ & $\uparrow$ $a_f$ &$\downarrow$ $b$    & $\downarrow$ $R^2$ & $\uparrow$ Acc    & $\downarrow$ $\Delta S$ & $\downarrow$ $\Delta G$ & $\uparrow$ lms & $\downarrow$ ss & $\uparrow$ ICAT  \\ \midrule
LLaMA 7B    & 0.235  & \bf{0.320} & 0.072  & 0.494 & {\bf 59.1\%} & 40.3\%     & 3.0\%      & 95.2       & 71.9       & 53.7      \\
DAMA      & \underline{\bf{-0.005}} & 0.038 & \underline{\bf{-0.006}} & \underline{\bf{0.208}} & 57.3\% & {\bf 31.5\%}     & 2.3\%      & 95.5       & {\bf 69.3} & {\bf 58.5}      \\
$\pm$ (std) & 0.004  & 0.004 & 0.004  & 0.026 & 0.5\%  & 0.9\%      & 0.7\%      & 0.3        & 0.8        & 1.5       \\
MEMIT      & 0.209  & 0.282 & 0.071  & 0.497 & 59.3\% & 40.5\%     & 3.3\%      &  \underline{95.6}       & 72.0       & 53.6      \\
% +FT         &        &       &        &       &        &            &            &            &            &           \\ 
\midrule
LLaMA 13B   & 0.270  & \underline{0.351} & 0.070   & 0.541 & 70.5\% & 35.7\%     & -1.5\%     & 95.2       & 71.4       & 54.4      \\
DAMA       & 0.148  & 0.222 & 0.059  & 0.472 & 66.4\% & 31.1\%     & -1.1\%     & 94.4       & 68.6       & 59.4      \\ \midrule
LLaMA 30B   & 0.265  & 0.343 & 0.092  & 0.499 & 71.0\% & 36.0\%     & -4.0\%     & 94.7       & 68.4       & 59.9      \\
DAMA       & 0.105  & 0.172 & 0.059  & 0.471 & 63.7\% & \underline{26.7\%}     & -3.7\%     & 94.8       & \underline{65.7}     & \underline{65.0}      \\ \midrule
LLaMA 65B   & 0.249  & 0.316 & 0.095  & 0.490 & \underline{73.3\%} & 35.7\%     &  1.4\%     &   94.9     & 69.5       & 57.9      \\
DAMA       & 0.185  & 0.251 & 0.100  & 0.414 & 71.1\% & 27.2\%     &  \underline{0.8\%}     &   92.8     & 67.1       & 61.1    \\ \bottomrule
\end{tabular}
\caption{Bias evaluation for the \llama{} models and their debiased instances
Significance analysis for the 7B model was performed by running \dama{} with five random seeds.
We bold the score for the original model or \dama{}, whichever is better if there are more than two standard deviations apart. We underline the best value in each column.
% \martin{Unify the number of decimal digits reported in each column, right-align the columns and the decimal dot will be vertically aligned as it should be.}
}
\label{tab:main-results-bias}
\end{table}

==> tables/main_results_old.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{@{}l|cccc|ccc|c||ccc|ccc@{}}

\toprule
          & \multicolumn{4}{c|}{Bias in LM} & \multicolumn{3}{c||}{WinoBias} & LM& \multicolumn{3}{c|}{StereoSet (gen)} & \multicolumn{3}{c}{Downsteram} \\
          & $a_s$     & $a_f$     & $b$  & $R^2$  & Acc  & $\Delta S$    & $\Delta G$   & PPL & LM        & ss        & ICAT        & ARC-C      & MMLU      & OBQA     \\ \midrule
LLaMA 7B  &  0.235   &  0.320   &    0.072       &   0.494        &  59.1\%      &  40.3\%   &   3.0\%            &     26.1         & 95.2      & 71.9      &             53.7        &  42.2     &           &    57.2  \\
+ DAMA    &  -0.005   &  0.038   &    -0.006       &   0.208        &   57.3\%     & 31.5\%    &     2.31\%          &    28.9       & 95.5      & 69.3      &             58.5        &  41.8     &           &    56.2   \\ % l9_on_nd256_ncv_val_neutral_delta_only_nw
$\pm$ (std)    & 0.004    &   0.004 &  0.004  &    0.026    & 0.5\%       &  0.9\%  &   0.7\%      &     0.2         & 0.3  & 0.8 &        1.5   & 0.4    &           &     0.5  \\
+MEMIT   & 0.209     &  0.282   &  0.071        &    0.497       &    59.3\%    &  40.5\%   &     3.3\%          &    26.1          & 95.6      & 72.0      &             53.6        &           &           &       \\
+FT      &      &      &           &           &        &     &               &              &           &           &             &           &           &       \\ \midrule
LLaMA 13B &     &     &           &           &        &     &               &              & 95.2      & 71.4      &             54.4        &  44.9     &           &    55.4   \\ 
+DAMA     &     &     &           &           &        &     &               &              & 94.4      & 68.6      &             59.4        &  44.7     &           &     56.2  \\\midrule%l11_on_nd512_ncv_val_neutral_delta_only_nw
LLaMA 30B &     &     &           &           &        &     &               &              & 94.7      & 68.4      &             59.9        &           &           &       \\
+DAMA    &      &     &           &           &        &     &               &              & 94.8      & 65.7      &             65.0        &            &           &       \\ \midrule % l17_on_ncv_val_neutral_delta_only_nw
LLaMA 65B &     &     &    ?        &           &        &     &               &              &           &           &             &            &           &       \\
+DAMA   &    &      &           &           &        &     &               &              &           &           &             &            &           &       \\ \bottomrule
\end{tabular}
\caption{Performance and bias evaluation for the \llama{} models and their debiased instances.}
\label{tab:main-results}
\end{table}

==> tables/main_results_performance.tex <==
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{@{}lccccc@{}}
\toprule
            & LM   & \multicolumn{4}{c}{Downstream} \\ \cmidrule(lr){2-2} \cmidrule(l){3-6}
            & $\downarrow$ PPL  & $\uparrow$ ARC-C     & $\uparrow$ ARC-E    & $\uparrow$ OBQA  & $\uparrow$ MMLU \\ \midrule
LLaMA 7B    & \bf{26.1} & 42.2      & \bf{69.1}    & 57.2  & 30.3 \\
DAMA      & 28.9 & 41.8      & 68.3     & 56.2  & 30.8 \\
$\pm$ (std) & 0.2  & 0.4       & 0.2      & 0.5   & 0.5  \\
MEMIT      & 26.1 & 42.7      & 68.9     & 57.0  &  30.2 \\ \midrule
% +FT         &      &           &          &       &      \\ \midrule
LLaMA 13B   & 19.8 & 44.9      & 70.6     & 55.4  & 43.3 \\
DAMA       & 21.0 & 44.7      & 70.3     & 56.2  & \underline{43.5} \\ \midrule
LLaMA 30B   & 20.5 & \underline{47.4}      & 72.9     & 59.2  & ---  \\
DAMA       & 19.6 & 45.2      & 71.6     & 58.2  & ---  \\ \midrule
LLaMA 65B   & \underline{19.5} & 44.5      & \underline{73.9}     & \underline{59.6}  & ---  \\
DAMA       & 20.1 & 40.5      & 67.7     & 57.2  & ---  \\  \bottomrule
\end{tabular}
\caption{Performance evaluation for the \llama{} models and their debiased instances. The significance analysis was performed as described in Table~\ref{tab:main-results-bias}.}
\label{tab:main-downstream}
\end{table}
